Opportunistic Communication in Extreme Wireless Sensor Networks

Sensor networks can nowadays deliver 99.9% of their data with duty cycles below 1%. This remarkable performance is, however, dependent on some important underlying assumptions: low traffic rates, medium size densities and static nodes. In this thesis, we investigate the performance of these same resource-constrained devices, but under scenarios that present extreme conditions: high traffic rates, high densities and mobility: the so-called Extreme Wireless Sensor Networks (EWSNs).

==> cv/cv.tex <==
\chapter*{Curriculum Vit\ae}
\addcontentsline{toc}{chapter}{Curriculum Vit\ae}
\setheader{Curriculum Vit\ae}

%% Print the full name of the author.
\makeatletter
\authors{\@firstname\ {\titleshape\@lastname}}
\makeatother

\noindent
\begin{tabular}{p{4\parindent}l}
    14-03-1879 & Born in Ulm, Germany.
\end{tabular}

\section*{Education}

\begin{tabular}{p{4\parindent}l}
    1892--1896 & Grammar School \\
    & Luitpold Gymnasium, M\"unich (1892--1895)\\
    & Aurau, Switzerland (1895--1896) \\
    \\
    1896--1900 & Undergraduate in Mathematics \& Physics \\
    & Eidgen\"ossische Polytechnische Schule Z\"urich \\
    \\
    1905 & PhD.\ Physics \\
    & Eidgen\"ossische Polytechnische Schule Z\"urich \\
    &
    %% The width of the second column is the width of the page, minus the width
    %% of the first column (4\parindent) minus four times the separation between
    %% the start of the column and its contents.
    \begin{minipage}{\textwidth-4\parindent-4\tabcolsep}
        %% We divide the minipage 20/80.
        \begin{tabular}{@{}p{0.2\linewidth}@{}p{0.8\linewidth-\tabcolsep}}
            \textit{Thesis:} & Eine neue Bestimmung der Molek\"uldimensionen \\
            \textit{Promotor:} & Prof.\ dr.\ A.\ Kleiner
        \end{tabular}
    \end{minipage}
\end{tabular}

\section*{Awards}

\begin{tabular}{p{4\parindent}l}
    1922 & Nobel Prize in Physics \\
    \\
    1925 & Copley Medal \\
    \\
    1929 & Max Planck Medal \\
    \\
    1999 & Time magazine's person of the century
\end{tabular}

\section*{Selected Publications}

\begin{itemize}
\item Leveraging Proximity Sensing to Mine the Behavior of Museum Visitors
Claudio Martella, Armando Miraglia, Marco Cattani, Maarten van Steen (PERCOM 2016) – Best paper runner-up

\item Graph Scale-Space Theory for Distributed Peak and Pit Identification
Andres Loukas, Marco Cattani, Marco Zuniga, Jie Gao (IPSN 2015)

\item Lightweight neighborhood cardinality estimation in dynamic wireless networks Marco Cattani, Marco Zuniga, Andres Loukas, Koen langendoen (IPSN 2014) – Best paper runner-up

\item SOFA: Communication in Extreme Wireless Sensor Networks
Marco Cattani, Marco Zuniga, Matthias Woehrle, Koen Langendoen (EWSN 2014)

\item Think Globally, Act Locally: On the Reshaping of Information Landscapes 
Andreas Loukas, Marco Zuniga, Matthias Woehrle, Marco Cattani, Koen Langendoen (IPSN 2013)

\end{itemize}



==> problem/problem.tex <==
%!TEX root = ../dissertation.tex

\chapter{Problem statement}
\label{chapter:problem}

- intro to wsn vs ewsn characteristics

% DUTY CYCLE

The constrained energy resources of WSN led to a first generation of protocols
that traded bandwidth utilization for lower energy consumption. Such protocols are based on asynchronous radio duty-cycling methods, which implies that senders need to wait for their receiver to wake up (to rendezvous), before sending their data. While in low power listening (LPL)~\cite{buettner:2006} nodes send a beaconing sequence until the receiver wakes up, in low power probing (LPP)~\cite{Dutta:2010,sun:2008}, the sender waits for a wakeup beacon from the receiver.  
%Despite their high overhead (most of the bandwidth is used for coordination purposes and not for data transmission), these protocols work well in traditional WSN, where the data rate is low (few senders, many receivers). 
%With a wakeup period of 200 ms, for example, the rendezvous phase of LPL protocols will last on average 100 ms~\footnote{In LPL, it is well known that the expected duration of an encounter takes half of the wake period~\cite{buettner:2006,Moss:2008}}. A lot more than the few millisecond needed for the data communication. In the best scenario, this will allows no more than 20 nodes to transmit their data every 2 seconds. Beyond this threshold, the channel saturates. 

The WSN community is well aware of the limitations of the first generation of low-power protocols and several notable contributions have improved their performance. To reduce the overhead of the rendezvous phase, protocols such as WiseMAC~\cite{Hoiydi:2004} keep track of the wakeup periods of their neighbors and use this information to wakeup just a few instants before the intended receiver. This type of protocols works very well on stable networks, where the overhead of estimating the wake periods is seldom done. Highly mobile scenarios, however, prevent the use of these methods. 

Another efficient way to disseminate information has been recently proposed by Ferrari et al.~\cite{Ferrari:2012}. By using a finely synchronized TDMA mechanism, together with extremely efficient network-wide floods, the authors are able to disseminate information irrespective of mobility.  However, their low-power wireless bus requires a central coordinator and a network with limited diameter (the synchronization degrades as the number of hops increases). The wide scale (graph diameter) of EWSN prevents the use of this approach, and the central coordinator exposes a single point of failure.
%Another line of relevant studies is cross-layer approaches, such as IRIS~\cite{Camillo2013} and XLP~\cite{Vuran2010}. Cross-layer solutions aim at creating more cohesive and specialized network stacks to overcome the challenges of particular scenarios. These solutions, however, rely on legacy MAC protocols such as CSMA/CA, and on legacy routing techniques such as gradients, and they are not suitable to work under extreme conditions. 

% communication over DC (synch vs asynch)
% lpl vs, lpp
% unicast and broadcast

% ewsn


% CHALLENGES, where things break

From a networking perspective, communication in mobile scenarios with high traffic rates and high densities poses several non-trivial technical challenges. First, similar to traditional WSN, these Extreme Wireless Sensor Networks (EWSN) also work with devices with limited energy resources and need to rely on radio duty-cycling techniques to save energy. Second, due to the network scale and node mobility, we cannot rely on methods that combine duty cycling techniques with central coordinators~\cite{Ferrari:2012} or that require some level of synchronization between the wake up periods of a given node and its neighbors~\cite{Hoiydi:2004,Tang:2011}. The system must be asynchronous and fully distributed. Third, due to their inefficient bandwidth utilization, traditional unicast and broadcast primitives --which are asynchronous, distributed and built on top of duty cycling techniques~\cite{buettner:2006,sun:2008}-- simply collapse under the traffic-demands of EWSN.

Unfortunately, from a networking perspective, communication in mobile scenarios with high traffic rates and high densities poses three non-trivial technical challenges.

\% paragraph{Energy efficiency.}
First, similar to traditional Wireless Sensor Networks (WSN), these \emph{Extreme Wireless Sensor Networks} (EWSN) also need to work with limited energy resources (small batteries or super-capacitors) and must rely on a number of techniques to save energy. The most common, \emph{radio duty-cycling}, consist in using the radio only periodically and for very short periods (few milliseconds). Since the radio is usually one of the most energy demanding component, a low ratio between the radio activity time and the stand-by time allows to extend the lifetime of sensor devices up to 100 times. (expand duty cycle, add graph).
Unfortunately, duty cycling the radio has two main drawbacks: limits the amount of information senses by the radio and and makes the devices' rendezvous more difficult. (explain better)

%Unfortunately, this also limits the time available to the wireless devices for exchanging information.

%After almost 25 years, the topic of Wireless Sensor Networks produced several hardware platforms\cite{} and operating systems~\cite{} running many communication protocols, each specifically designed for its application scenario. While being all different, mosto of these protocols share the same energy-saving mechanism called Radio Duty Cycling. With this technique, device are able to enxtend their lifetime up to 2 order of magnitude.


\paragraph{Robustness.}
Second, due to the network scale and node mobility, we cannot use methods that rely on a central coordinators or that require some level of synchronization between the activity time of devices. The already limited bandwidth cannot be contraine to a small subset of time or be saturated with synchronization messages. Moreover connectivity cannot be guaranteed all the time (add the problem of node drifting)(add special problem of synchronization in proximity detection where, due to the short range of devices, diameter is usually large and network and nodes can be often disconnected). Therefore, the system must be asynchronous and fully distributed.

\paragraph{Scaling.}
Third, due to their inefficient bandwidth utilization, traditional unicast and broadcast communication primitives –which are asynchronous, distributed and built on top of duty cycling techniques– simply collapse under the extreme demands and dynamics of EWSN.


Henceforth, providing an energy-efficient stack for communicating in EWSN requires a careful evaluation of the following problem: in asynchronous duty cycling techniques, much of the bandwidth is wasted in coordinating the rendezvous of the (sleeping) nodes. In EWN, nodes need to reduce this overhead to free up the channel’s bandwidth for actual data transmissions.





%To our possibility, in this thesis we aim at removing some of WSN's limitations and make a concrete step towards the smart dust dream. In particular, we target networks that are xxxxxx and, for these reasons, defined as EWSN




==> publications/publications.tex <==
%!TEX root = ../dissertation.tex
\chapter*{List of Publications}
\addcontentsline{toc}{chapter}{List of Publications}
\setheader{List of Publications}
\label{publications}

%% We use the 'etaremune' environment (the reverse of 'enumerate') to get a
%% numbered list of publications in reverse chronological order. If the list of
%% authors is long, it might be useful to emphasize your own name with \textbf.
\begin{enumerate}\small{

\item \textbf{M. Cattani}, M. Zuniga, M. Woehrle, K.G. Langendoen, \textit{SOFA: Communication in Extreme Wireless Sensor Networks}, in \textit{11th European Conference on Wireless Sensor Networks (EWSN)} (2014)

\item \textbf{M. Cattani}, M. Zuniga, A. Loukas, K.G. langendoen, \textit{Lightweight neighborhood cardinality estimation in dynamic wireless networks}, in \textit{13th ACM/IEEE International Conference on Information Processing in Sensor Networks (IPSN)} (2014)

\item \textbf{M. Cattani}, A. Loukas,  M. Zimmerling, M. Zuniga, K. Langendoen, \textit{Staffetta: Smart Duty-Cycling for Opportunistic Data Collection}, in \textit{14th ACM Conference on Embedded Networked Sensor Systems (SenSys)} (2016).

\item A. Loukas, M. Zuniga, M. Woehrle, \textbf{M. Cattani}, K.G. Langendoen, \textit{Think Globally, Act Locally: On the Reshaping of Information Landscapes}, in \textit{12th International Conference on Information Processing in Sensor Networks (IPSN)} (2013)

\item A. Loukas, \textbf{M. Cattani}, M. Zuniga, J. Gao, \textit{Graph Scale-Space Theory for Distributed Peak and Pit Identification}, in \textit{14th ACM/IEEE International Conference on Information Processing in Sensor Networks (IPSN)} (2015)

\item C. Martella, A. Miraglia, \textbf{M. Cattani}, M. van Steen, \textit{Leveraging Proximity Sensing to Mine the Behavior of Museum Visitors}, in \textit{IEEE International Conference on Pervasive Computing and
Communications (PerCom)} (2016).

}

\end{enumerate}

